fAux: Testing Individual Fairness via Gradient Alignment

Machine learning models are vulnerable to biases that result in unfair treatment of individuals from different populations. Recent work that aims to test a model's fairness at the individual level either relies on domain knowledge to choose metrics, or on input transformations that risk generating out-of-domain samples. We describe a new approach for testing individual fairness that does not have either requirement. We propose a novel criterion for evaluating individual fairness and develop a practical testing method based on this criterion which we call fAux (pronounced fox). This is based on comparing the derivatives of the predictions of the model to be tested with those of an auxiliary model, which predicts the protected variable from the observed data. We show that the proposed method effectively identifies discrimination on both synthetic and real-world datasets, and has quantitative and qualitative advantages over contemporary methods.

==> bonus_material.tex <==
To further investigate the performance gap between FTA and fAux, we show the scatter plots~(see Figure \ref{fig:corr-plots}) side by side for the Synthetic-8 scenario in Table \ref{table:synth-data-res}. Given an unfair model whose predictions are denoted as white circles, we note both FTA and fAux+IG show a positive correlation between ground truth fairness labels (y-axis) and predictions (x-axis). 
%\Simon{I do not see a strong positive correlation!} 
% addressed by updating figure
This observation indicates both of the approaches are effective in terms of flagging discrimination. However, given a guaranteed fair model whose predictions are denoted as black crosses, we note the FTA mistakenly flags many individual unfair treatments. This reflects our previous comment in Section~\ref{sec:existing_approaches}: FTA may identify models that lack adversarial robustness as unfair, which mistakenly mixes up the two types of safety criteria. Please refer to Appendix~\ref{sec:discussion_relation_ar} to see the relation between adversarial robustness and fairness testing.

\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.49\linewidth}
     \centering
        \includegraphics[width=\textwidth]{figs/relabelled_ynorms.pdf}
        \caption{FTA}
        \label{fig:corr:fta}
     \end{subfigure}
     \hspace{\fill}
     \begin{subfigure}[b]{0.49\linewidth}
     \centering
        \includegraphics[width=\textwidth]{figs/relabelled_int_aux_test.pdf}
        \caption{fAux+IG}
        \label{fig:corr:int}
     \end{subfigure}
    %  \hspace{\fill}
    %  \begin{subfigure}[b]{0.32\linewidth}
    %     \includegraphics[width=\textwidth]{figs/true_grad_test.pdf}
    %     \caption{LIC-UB}
    %     \label{fig:corr:true}
    %  \end{subfigure}
    %  \hspace{\fill}
    %  \begin{subfigure}[b]{0.24\linewidth}
    %     \includegraphics[width=\textwidth]{figs/fliptest.pdf}
    %     \caption{Fliptest}
    %     \label{fig:corr:fliptest}
    %  \end{subfigure}
    %  \hspace{\fill}

    \caption{\textbf{Prediction vs Ground-truth IFS.} Comparing the alignment of the ground-truth discrimination score and the scores of different fairness tests. White circles denote individuals treated by an unfair model. Black crosses denote individuals treated by a model that's constrained to be fair.   While both tests show agreement with the ground truth for unfair models, FTA outputs a high discrimination score even for individuals that experience no discrimination. In contrast, these individuals receive a low discrimination score from fAux (collapsing to a point in (b)).
    %The black crosses correspond to individuals passed through a model constrained to be fair, whereas the white circles correspond to an unconstrained model. 
    }
    \label{fig:corr-plots}
\end{figure}

==> connect_earlier_notions_of_ind_fairness.tex <==
This connects the earlier notions of individual fairness: 
\begin{itemize}[leftmargin=10pt, noitemsep]
    \item {\bf Fairness through unawareness:} The refined definition is related to FTU in that it stipulates models be insensitive to changes in protected variables. However unlike FTU, it is aware of the influence of the protected variables on the features.
    \item {\bf Fairness through awareness:} The refined definition belongs to the family of FTA as it provides concrete input and output similarity metrics; it states that an arbitrary change in the latent variable $\mathbf{z}_{\parallel}$ should result in a negligible change in the output  $f_{tar}(\mathbf{x}_{i})$.
    %Our definition is framed in terms of distances of inputs and outputs; an arbitrary change in the latent variable $\mathbf{z}_{\parallel}$ should result in a negligible change in the output  $f_{tar}(\mathbf{x}_{i})$.

     \item {\bf Counterfactual fairness:} The refined definition leverages a generative model, and tests model fairness by modifying latent variables that are correlated with protected variable. 
   
    %The function $f_{tar}(\mathbf{x}_{i})$ does not explicitly use the protected variables $\mathbf{c}$.
\end{itemize}

==> limitations_of_ftu_and_fta.tex <==
\subsection{Limitations of Existing Definitions}\label{sec:limitations}
\label{sec:existing_approaches}

There are many reasons why models exhibit discriminatory behaviour \citep{mehrabi2019survey,FrameworkForBias}, but one of the most common is the mishandling of {\em historical bias} in the training data~\citep{fuchs2018dangers}.  Here, pre-existing prejudices create a misalignment between the collected data and the goals of the model \citep{FrameworkForBias} and models may learn to propagate this bias via their decisions. Figure~\ref{fig:pgm_data} shows the potential data generation graph, where the label $Y$ and protected attributes $C$ may (or may not) correlate due to the historical bias. A fair model~(Figure~\ref{fig:pgm_fair}) would learn to infer label $Y$ by disentangling the impact from the protected variables $C$. In contrast, an unfair model~(Figure~\ref{fig:pgm_unfair}) implicitly infers the protected variables to support its prediction of the label $Y$.

The limitations of the FTU and FTA approaches are easily understood in terms of this graphical model.  Models that meet the FTU definition are not guaranteed to be fair~\citep{FairMLBook} since they overlook correlation between features $X$ and protected variables $C$.  Discrimination persists when the feature becomes a {\em surrogate} for the protected variables.  We might expect tests based on the FTU to have low recall since they are insensitive both to the protected variable and to discrimination induced by these surrogates. Tests based on FTA potentially have the opposite problem;  they are sensitive to both unfairness induced directly by the protected variable and indirectly via surrogate features. However, since these tests are based on distance metrics, they are also sensitive to other changes such as adversarial examples in which a small change in the input can create a large change in the prediction.  Hence, we might expect them to have low precision. We illustrate these limitations in Section \textit{Use Cases} of the supplementary materials.
%with some use cases.

With access to a causal generative model, CFF can recognize surrogate features and the decisions that result from them.  However, training such models with unsupervised learning is hard \citep{ImprovedGANTechniques,ReducingModeCollapse} and the testing procedure can produce misleading conclusions if the generative model is ill-defined or inaccurate. 

\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.32\linewidth}
     \centering
        \includegraphics[width=0.8\textwidth]{figs/pgm_data.pdf}
        \caption{Data Generation}
        \label{fig:pgm_data}
     \end{subfigure}
     \hspace{\fill}
     \begin{subfigure}[b]{0.32\linewidth}
     \centering
        \includegraphics[width=0.8\textwidth]{figs/pgm_fair.pdf}
        \caption{Fair Model}
        \label{fig:pgm_fair}
     \end{subfigure}
     \hspace{\fill}
    \begin{subfigure}[b]{0.32\linewidth}
    \centering
        \includegraphics[width=0.8\textwidth]{figs/pgm_unfair.pdf}
        \caption{Unfair Model}
        \label{fig:pgm_unfair}
     \end{subfigure}
        \caption{\textbf{Graphical models to show how historical bias causes unfairness.} (a) Generation process of a biased training dataset.The red dashed line denotes that $Y$ and $C$ may have correlations due to historical bias. (b) Fair models learn to infer $Y$ while cancelling the impact from protected variables $C$. Solid arrows show generative dependence. Dashed arrow shows learned inference mapping. (c) Unfair models infer the protected variables to support their predictions.}
        \label{fig:graphical-models}
\vspace{-5mm}
\end{figure}


%More First, it can be difficult to define distance metrics. For example, measuring the semantic distance between natural language sentences is challenging.  Second, when a data point $(\mathbf{x}, y)$ violates FTA, it is hard to determine whether this is unfairness  or just a lack of adversarial robustness. 



%the model may fulfill its training objective by exploiting correlations between the target variable $Y$ and protected variables $C$, even when %the protected variables are not present during the model training. More precisely, the target model $f_{tar}$ learns the prediction mapping %between feature attributes $X$ and label $Y$ by implicitly inferring the protected attributes $C$. 


%Existing approaches to test for individual fairness are limited by their associated definition. 

%Verification based on the FTA definition is also limited for two reasons. First, it can be difficult to define distance metrics. For example, %measuring the semantic distance between natural language sentences is challenging.  Second, when a data point $(\mathbf{x}, y)$ violates FTA, it %s hard to determine whether this is unfairness  or just a lack of adversarial robustness. 
%\Christopher{can we expand a bit on this second drawback? its not clear was is meant by lack of robustness here and how this can make it hard to distinguish unfairness (maybe an example?).}
% wuga: not sure if it is sufficient, but I changed the lack of robustness to lack of adversarial robustness.

%The limitations of both of these approaches are revealed when considering \textit{historical bias}. Here, pre-existing prejudices create a misalignment between the collected data and the goals of the model \citep{FrameworkForBias} and models may learn to propagate this bias via their decisions.  FTU may enforce this bias, because patterns in the observed data $X$ may act as surrogates for the protected variable.  Depending on the metric, FTA may not be able to distinguish between these patterns of bias and other modelling errors.


%Moreover, training a generative model is a difficult task \citep{ImprovedGANTechniques,ReducingModeCollapse}. 

%\Christopher{In the definition of CFF in section 2.2.3, it's not clear where the generative model is used, can we clarify this in that section so that it make more sense when you mention it here?} 
% wuga: yup, done


==> previous_definitions_of_fairness.tex <==
\subsection{Previous definitions}
\label{sec:multiple_individiual_fairness_definitions}
By individual fairness, we mean the tolerable discrepancy of model predictions at an individual level (i.e., for one data point).  This can reveal hidden unfairness that can't be identified at an aggregate level using a group fairness criterion. The three most widely used definitions that operate at this level are as follows:% \cite[see][for others]{mehrabi2019survey}.

%%MODIFIED FROM ORIGINAL

%(see ~\footnote{We note there are more definitions for individual fairness in the literature~\cite{mehrabi2019survey}}.
%\subsubsection{Fairness Through Unawareness}
\textbf{Fairness Through Unawareness}~(FTU) states that:

\textit{A predictor is said to achieve fairness through unawareness if protected attributes are not explicitly used in the prediction process.}

A model can satisfy the FTU definition by either excluding the protected attributes $C$ as input during training or by ensuring that perturbations to $C$ do not affect predictions.

%\cite{galhotra2017fairness} proposed to diagnose potential discrimination in the %\Christopher{model (replaces "software")} 
% the paper used the term of "software"
%software based on the FTU definition.
%\Simon{I agree that software reads really weirdly here.  I'd go with model.}

%\subsubsection{Fairness through Awareness}
\textbf{Fairness Through Awareness}~(FTA) states that: \textit{
Similar individuals should be treated similarly.
%\Christopher{Similar individuals should be treated similarly. (replaces rest of italics)} 
% wuga: the paper stated the sentence below actually.
%Treating similar individuals similarly.
}
Given two observations $(\mathbf{x}_i,y_i)$ and $(\mathbf{x}_j,y_j)$, a model $f_{tar}$ satisfies this definition when the Lipschitz property holds:
\begin{equation}
    \phi_{out}(f_{tar}(\textbf{x}_i), f_{tar}(\textbf{x}_j)) \leq \phi_{in}(\textbf{x}_i, \textbf{x}_j), 
    \label{eq:metric-fta}
\end{equation}
where $\phi_{in}(\cdot,\cdot)$ and $\phi_{out}(\cdot,\cdot)$ are distance metrics in the input and output spaces.  

%\cite{john2020verifying} used formal verification to validate models based on this definition. Likewise, \cite{wachter2017counterfactual} used %adversarial attacks to search for violations. 

%\subsubsection{Counterfactual Fairness}
\textbf{Counterfactual Fairness}~(CFF) stipulates that prediction variables $Y$ should not causally depend on protected variables $C$ when holding other features $X$ constant.

Given observed feature $\mathbf{x}$, prediction $y$ and protected variables $\mathbf{c}$, counterfactual fairness holds if:
\begin{equation}
    P(y|\mathbf{x},\mathbf{c}) = P_{C\leftarrow\textit{do}(\mathbf{c}')}(y| \mathbf{x}, \mathbf{c}), 
\end{equation}
where the $do(\cdot)$ operation~\cite{pearl2009causal} changes protected attributes from $\mathbf{c}$ to $\mathbf{c}'$ during inference. To apply this operation, we need a generative model that explicitly describes the causal structure of the variables.
%\Christopher{why do we need this "do" operator? can't we put $c'$ directly in the right hand side of the equation and remove $C\leftarrow\textit{do}(\mathbf{c}')$?}
% wuga: "do" operation is not simple replacement, the above equation is on counterfactual inference. :)


% Hmmm... lets think about commenting the below as the FlipTest had given a good description. We just need to refer to them, if space is limited. No action for now until the paper is in a good shape.

%FlipTest~\cite{black2019fliptest}, is based on counterfactual fairness. %The authors construct \textit{flipsets} $S_{flip}$, which comprise (instance, counterfactual) pairs $(\textbf{x}, \textbf{x}^{\prime})$ for which the target model $f_{tar}$ predicts different labels. The difference between these pairs are aggregated into \textit{transparency reports} that highlight features that are responsible for the differences in prediction.  

% The transparency report is defined as:

% \begin{equation}
%     \frac{1}{|S_{flip}|}\sum_{x, x^{\prime} \in S_{flip}} (\textbf{x} - \textbf{x}^{\prime}). \label{eq:transparency-report-fliptest-og}
% \end{equation}

% Sorting this vector by absolute value defines a ranking over the features where higher ranking features correspond to surrogates for protected group membership. 

% Consider to not mention the limitations, since you are not claiming it as contribution -Wuga
%------------------------------------
% \subsection{Limitations}\label{sec:limitations}
% \label{sec:existing_approaches}

% There are many reasons why models exhibit discriminatory behaviour \cite{mehrabi2019survey,FrameworkForBias}, but one of the most common is the mishandling of {\em historical bias} in the training data~\cite{fuchs2018dangers}.  Here, pre-existing prejudices create a misalignment between the collected data and the goals of the model \cite{FrameworkForBias} and models may learn to propagate this bias via their decisions. Figure~\ref{fig:pgm_data} shows the potential data generation graph, where the label $Y$ and protected attributes $C$ may (or may not) correlate due to the historical bias. A fair model~(Figure~\ref{fig:pgm_fair}) would learn to infer label $Y$ by disentangling the impact from the protected variables $C$. In contrast, an unfair model~(Figure~\ref{fig:pgm_unfair}) implicitly infers the protected variables to support its prediction of the label $Y$.

% The limitations of the FTU and FTA approaches are easily understood in terms of this graphical model.  Models that meet the FTU definition are not guaranteed to be fair~\cite{FairMLBook} since they overlook correlation between features $X$ and protected variables $C$.  Discrimination persists when the feature becomes a {\em surrogate} for the protected variables.  We might expect tests based on the FTU to have low recall since they are insensitive both to the protected variable and to discrimination induced by these surrogates. Tests based on FTA potentially have the opposite problem;  they are sensitive to both unfairness induced directly by the protected variable and indirectly via surrogate features. However, since these tests are based on distance metrics, they are also sensitive to other changes such as adversarial examples in which a small change in the input can create a large change in the prediction.  Hence, we might expect them to have low precision. We illustrate these limitations in Section \textit{Use Cases} of the supplementary materials.
% %with some use cases.

% With access to a causal generative model, CFF can recognize surrogate features and the decisions that result from them.  However, training such models with unsupervised learning is hard \cite{ImprovedGANTechniques,ReducingModeCollapse} and the testing procedure can produce misleading conclusions if the generative model is ill-defined or inaccurate. 
% ----------------------------

\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.32\linewidth}
     \centering
        \includegraphics[width=0.8\textwidth]{figs/pgm_data.pdf}
        \caption{Data Generation}
        \label{fig:pgm_data}
     \end{subfigure}
     \hspace{\fill}
     \begin{subfigure}[b]{0.32\linewidth}
     \centering
        \includegraphics[width=0.8\textwidth]{figs/pgm_fair.pdf}
        \caption{Fair Model}
        \label{fig:pgm_fair}
     \end{subfigure}
     \hspace{\fill}
    \begin{subfigure}[b]{0.32\linewidth}
    \centering
        \includegraphics[width=0.8\textwidth]{figs/pgm_unfair.pdf}
        \caption{Unfair Model}
        \label{fig:pgm_unfair}
     \end{subfigure}
        \caption{\textbf{Graphical models to show how historical bias causes unfairness.} (a) Generation process of a biased training dataset.The red dashed line denotes that $Y$ and $C$ may have correlations due to historical bias. (b) Fair models learn to infer $Y$ while cancelling the impact from protected variables $C$. Solid arrows show generative dependence. Dashed arrow shows learned inference mapping. (c) Unfair models infer the protected variables to support their predictions.}
        \label{fig:graphical-models}
\vspace{-5mm}
\end{figure}


%More First, it can be difficult to define distance metrics. For example, measuring the semantic distance between natural language sentences is challenging.  Second, when a data point $(\mathbf{x}, y)$ violates FTA, it is hard to determine whether this is unfairness  or just a lack of adversarial robustness. 



%the model may fulfill its training objective by exploiting correlations between the target variable $Y$ and protected variables $C$, even when %the protected variables are not present during the model training. More precisely, the target model $f_{tar}$ learns the prediction mapping %between feature attributes $X$ and label $Y$ by implicitly inferring the protected attributes $C$. 


%Existing approaches to test for individual fairness are limited by their associated definition. 

%Verification based on the FTA definition is also limited for two reasons. First, it can be difficult to define distance metrics. For example, %measuring the semantic distance between natural language sentences is challenging.  Second, when a data point $(\mathbf{x}, y)$ violates FTA, it %s hard to determine whether this is unfairness  or just a lack of adversarial robustness. 
%\Christopher{can we expand a bit on this second drawback? its not clear was is meant by lack of robustness here and how this can make it hard to distinguish unfairness (maybe an example?).}
% wuga: not sure if it is sufficient, but I changed the lack of robustness to lack of adversarial robustness.

%The limitations of both of these approaches are revealed when considering \textit{historical bias}. Here, pre-existing prejudices create a misalignment between the collected data and the goals of the model \cite{FrameworkForBias} and models may learn to propagate this bias via their decisions.  FTU may enforce this bias, because patterns in the observed data $X$ may act as surrogates for the protected variable.  Depending on the metric, FTA may not be able to distinguish between these patterns of bias and other modelling errors.


%Moreover, training a generative model is a difficult task \cite{ImprovedGANTechniques,ReducingModeCollapse}. 

%\Christopher{In the definition of CFF in section 2.2.3, it's not clear where the generative model is used, can we clarify this in that section so that it make more sense when you mention it here?} 
% wuga: yup, done


==> related_work.tex <==
\subsection{Limitations}

At a high level, many existing tests of individual fairness have the following general form:
\begin{enumerate}
    \item Select metrics on the input and output space $\phi_{in}$ and $\phi_{out}$.
    \item For each test point $\textbf{x}_i$ in the validation set, search for a point $\textbf{x}_j$ that satisfies $\phi_{in}(\textbf{x}_i, \textbf{x}_j) < \epsilon$.
    \item The maximum value of $\phi_{out}(f_{tar}(\textbf{x}_i), f_{tar}(\textbf{x}_j))$ measures the amount of discrimination experienced by $\textbf{x}_i$ under $f_{tar}$.
\end{enumerate}

\noindent We may thus compare tests according to how they approach steps (1) and (2).  With respect to the first step, the original FTA paper \citep{dwork2012fairness} requires task-specific metrics.  In the absence of domain knowledge, several works describe data-driven alternatives. For example, \cite{ilvento2020metric} uses an expert to classify certain pairs of inputs as similar, and then uses a metric-learning algorithm. Alternatively, \cite{Lahoti_2019} and \cite{mukherjee2020simple} proposed to use Metric learning. Some works make use of unweighted $l_p$ norms \citep{wachter2018counterfactual, john2020verifying}, though others obtain weights from a linear model trained to predict the protected variable $c$ from the input $\mathbf{x}$ \cite{ruoss2020learning,yurochkin2020training}. While fAux also learns its own metric, it does so in a principled fashion; its metric is derived directly from the LIC. Moreover, the auxiliary model used by fAux is more expressive than the linear models used by earlier works. Thus, the weights learned by fAux are non-uniform, and capture non-linear relationships between $x$ and $c$.  In our experiments, we show the benefit of the non-linearity.

For the second step, one line of work considers generating test points using adversarial techniques~\cite{wachter2018counterfactual,Ustun_2019,maity2021statistical}.  
%Given a individual $\mathbf{x}_i$, gradient ascent is performed on $\phi_{out}(f_{tar}(\textbf{x}_i), f_{tar}(\textbf{x}_j))$ to find an input $\mathbf{x}_j$ in the neighbourhood of $\mathbf{x}_i$.  
Unfortunately, these approaches have the potential to construct unrealistic, out-of-distribution samples, which may generate misleading conclusions. An alternative technique is to use the metric $\phi_{in}$ to compute the pairwise-similarity between all individuals, and then use Optimal Transport (OT) to define a mapping between protected groups~\cite{dwork2012fairness, pmlr-v97-gordaliza19a}. The resulting map can then be used to produce test inputs $\mathbf{x}_j$ for a given input $\mathbf{x}_i$. This approach has the advantage that the pairs considered are always real samples that come from the validation dataset. However, for large, high-dimensional datasets, OT can be computationally demanding, and also unstable. To this end, approximate methods, based on dual-formulations \cite{chiappa2021fairness} and Generative Adversarial Networks \citep{black2019fliptest} have also been explored. However, stochastic approximations may still be unstable, and may also inadvertently generate out-of-distribution samples. fAux, in contrast, avoids many of these disadvantages; it uses only supervised learning to train the auxiliary model, and only a single backward pass is required to perform the test. Thus, it scales well to high-dimensional problems. Moreover, it is a local test that is conducted only on in-distribution points.


==> reproducibility_checklist.tex <==
\section{Reproducibility Checklist}

\begin{enumerate}

\item This paper clearly states what claims are being investigated.
\textbf{Yes}.  Our contributions are outlined in the introduction.

\item This paper explains how the results substantiate the claims.
\textbf{Yes}.

\item This paper explicitly identifies limitations or technical assumptions.
\textbf{Yes}.  These are identified throughout the work, and are also summarized in the section \textit{Scope of Work} in the supplementary materials.

\item This paper includes a conceptual outline and/or pseudocode description of AI methods introduced.
\textbf{Yes}.  Pseudocode for the fAux test and synthetic dataset generation can be found, respectively, in Algorithms 1 and 2 of the supplementary materials.

\item Does this paper make theoretical contributions?
\textbf{Yes}.  We propose the \textit{Local Independence Criterion} (LIC) as a sufficient criterion for violation of our individual fairness, provided in Definition 1.  

\item All assumptions and restrictions are stated clearly and formally.
\textbf{Yes}.  These are summarized in the section \textbf{Scope of Work} in the supplementary materials.

\item All novel claims are stated formally (e.g., in theorem statements).
\textbf{Yes}.

\item Proofs of all novel claims are included.
\textbf{Yes}.  They are included in the supplementary materials.

\item Proof sketches or intuitions are given for complex and/or novel results.
\textbf{Yes}.  We provide both illustration and intuition for our model-inversion approximation in the section \textit{Using Pseudoinverses for Model Inversion} of the supplementary materials.

\item Appropriate citations to theoretical tools used are given.
\textbf{Yes}.

\item Does this paper rely on one or more data sets?
\textbf{Yes}.

\item All novel datasets introduced in this paper are included in a data appendix.
\textbf{Not applicable}

\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.
\textbf{Not applicable}.

\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textbf{Yes}.

\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available.
\textbf{Yes}.  

\item All datasets that are not publicly available are described in detail.
\textbf{Not applicable}.

\item Does this paper include computational experiments?
\textbf{Yes}.

\item All source code required for conducting experiments is included in a code appendix.
\textbf{No}.  

\item All source code required for conducting experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.
\textbf{No}. The description in the paper is sufficient to reproduce the code.

\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results.
\textbf{Yes}.  These details, and others, are described in the section \textit{Hyperparameters for the Fairness Tests.}

\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks.
\textbf{Yes.}

\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics.
\textbf{Yes}.  This is done in-depth in the section \textit{Evaluating Fairness Tests and Selecting $\delta$}.

\item This paper states the number of algorithm runs used to compute each reported result.
\textbf{Yes}.

\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information.
\textbf{Yes}.  We re-run our experiments on synthetic datasets with different collections of the hyperparameters, empirically measure variation by computing standard deviation.  Additionally, for the experiments on real datasets, we instead look at how the entire distribution of scores (visualized via histograms) for a given fairness tests changes when we compare fair and unfair models.

\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments.
\textbf{Yes}.

\item This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting.
\textbf{Yes}.

\end{enumerate}

==> todo.tex <==
* add in stuff without formatting
* add in stuff from openreview
* reformat
* how to add in supplementary materials?
* test compilation
* where to submit?
* copyright form
* complete checklist

* Ethical statement
* Optional acknowledgements




\input{introduction}
\input{notation_and_preliminary}
\input{methodology}
\input{experiment}
\input{conclusion}
\bibliographystyle{plain}
\bibliography{references}
\newpage
\input{checklist}
\newpage
\input{appendix}
\end{document}



Papers must be formatted in AAAI two-column, camera-ready style; see the AAAI-22 author kit for details. Papers must be in trouble-free, high-resolution PDF format, formatted for US Letter (8.5″ x 11″) paper, using Type 1 or TrueType fonts. AAAI submissions are anonymous, and must conform to the instructions for double-blind review (detailed under Review Process). The authors must manually remove all author and affiliation information from their submission for review, and may replace it with other information, such as paper number and keywords. Submissions may consist of up to 7 pages of technical content plus up to 2 additional pages solely for references; acknowledgements should be omitted from papers submitted for review, but may be included in these 2 additional pages for accepted papers. The AAAI copyright block is hard-coded into the AAAI paper templates to retain proper spacing and cannot be removed; however, it is not binding until a paper is accepted and a signed copyright form is submitted by the author.

-------------------

Works to cite:

More discussion here:
https://www.overleaf.com/project/610aa77510d5832697098073

[1] Yurochkin et al., 2019. Training individually fair ML models with sensitive subspace robustness.

[2] Xue et al., 2020. Auditing ML models for individual bias and unfairness.

[3] Maity et al., 2021. Statistical inference for individual fairness.




=====================

Related work:

* Other works that try to learn fairness metrics.  They provide ad hoc ideas.  In contrast, we derive a fairness metric from the local independence criterion.


* SenSei, https://arxiv.org/pdf/1905.10607.pdf other papers ... average individual fairness

* Adversarial testing strategies...Unfair Map


------------

Changelog:

* Rewrote abstract to remove descriptions of "verification"
* Remove Figure 3 (\label{fig:corr-plots})
* Change Definition 0.1
* Section on selecting delta
* Comparisons with Related Work section
* Added unfair map to experimental descriptions
* Updated FTA descriptions
* Removed primes from deltas
* 

TODO:

* URGENT: sections do not have numbering.  Therefore:
    4. Add in supplementary materials (in what form?)
    5. WHAT STEPS FOR SIMON???? [DONE]

[WUGA]
    1. Theorem numbers are weird; figure numbers are weird 
    2. Sections are not references.  Ex see the section describing the real datasets
    3. * Combine Table 2 and Table 3: score, #parameters, and training time.

[CODE]
    * Redo Figure (Factors that impact fAux performance)
    * Are you sure faux is calculated using abs values?
    * add in some real experiments (showing the adult use case)

[INTRO]
    * testing in the title seems somewhat misleading and it is not clear how to select a tolerance parameter

[RELATED WORKS]
    * [DONE] Add in missing works (see above)
	    - As we went through the papers you suggested, we notice most papers belong to the category of learning fairness metrics, which is different from our goal of fast individual fairness testing (potentially against given metrics). For example, `Metric Learning for Individual Fairness' paper uses an expert to classify certain pairs of samples as "similar," which is combined with metric learning in order to learn a similarity metric.
	    
    * [DONE] However, this notion of equal classification for similar individuals from different protected groups has already been considered by Ruoss et al. (2020) (denoted as Cat + Noise constraint). 
    
    * [DONE] Finally, while the paper claims that the proposed fairness notion does not require a similarity metric, this metric is implicitly encoded by the generative model (all individuals generated from varying the protected attribute)
    
    * [DONE] Overstate that the proposed method does not require a fair metric and correspondingly the weakness of other methods relying on the fair metric
    	- In terms of overstating `the proposed method does not require a fair metric', we want to clarify that we did not make this claim in our paper. Instead, we stated that the proposed approach does not require manually setting the metric since the proposed method uses derivatives (derived from the local independence criterion) to act as local fairness measurements.
    	- Unlike other approaches which suggest ad hoc metrics [citation], the local fairness criterion ...
    	
    * sensei...distributional individual fairness...
        * it is a model property, it is not an individual property.  Ie it cannot be used to test for individuals....
        
    * faux score combines everything together
    * principled? Rephrase, in intro
    
    * OT APPROACH CAN BE MADE THEORETICALLY RIGOROUS

[EXPERIMENT SECTION]
    * [Done] Update experimental setup section (ie candidate fairness testing algorithms)
    
    
    * Utility of the real data experiment. Why would anyone use fAux instead of directly computing mutual information on real data
    * Why is there a performance decline when data bias level is less than 0.25?
	    - Our hypothesis is that, when a target model is trained on less biased data, the target model is relatively fair on its predictions. Indeed, the accuracy of auxiliary model may be used to bound disparate treatment using an h-divergence [1]. Thus fAux loses its functionality since it cannot detect outstanding unfair treatments from a fair model.
    * Results exceed Local Independent Criterion Upper Bound (LIC-UB) [footnote?]
    
     Reviewer YkjV
    * [PARTIAL] Further, [13] does not consider unweighted norms, unlike claimed on L195.
        - I updated the description to show that it does.
        - I could find more papers to support this approach
    
    * compare with consistency score / kNN score?

    DONE:
        * Comment 3: negative values in figures
        
[DERIVATION]
    * [DONE] Comment 2: if  is a vector and  is scalar, then this may be a very bad estimate of x
    * Comment 1: target model is a function of both the training features as well as the training labels
    * [DONE] Comment 3: Regarding the arrow from Y to C [footnote].  
        - This is the generative model corresponding to the inference pat
        -SHOULD WE CHANGE THIS?
    * Comment 6: Regarding the transpose
    
    Reviewer YkjV
    * Furthermore, there are multiple errors, e.g., should be replaced by  in equations 9 to 11, ... the use of x0 instead of x


 

[Supplementary materials]
    Reviewer YkjV
    * Equation 26  should be , etc. ...




Material to include:


*


...


